Landmarking for Navigational Streaming of Stored High-Dimensional Media

Modern media data such as 360 videos and light field (LF) images are typically captured in much higher dimensions than the observers' visual displays. To efficiently browse high-dimensional media over bandwidth-constrained networks, a navigational streaming model is considered: a client navigates the large media space by dictating a navigation path to a server, who in response transmits the corresponding pre-encoded media data units (MDU) to the client one-by-one in sequence. Intra-coding an MDU (I-MDU) would result in a large bitrate but I-MDU can be randomly accessed, while inter-coding an MDU (P-MDU) using another MDU as a predictor incurs a small coding cost but imposes an order where the predictor must be first transmitted and decoded. From a compression perspective, the technical challenge is: how to achieve coding gain via inter-coding of MDUs, while enabling adequate random access for satisfactory user navigation. To address this problem, we propose landmarks, a selection of key MDUs from the high-dimensional media. Using landmarks as predictors, nearby MDUs in local neighborhoods are intercoded, resulting in a predictive MDU structure with controlled coding cost. It means that any requested MDU can be decoded by at most transmitting a landmark and an inter-coded MDU, enabling navigational random access. To build a landmarked MDU structure, we employ tree-structured vector quantizer (TSVQ) to first optimize landmark locations, then iteratively add/remove inter-coded MDUs as refinements using a fast branch-and-bound technique. Taking interactive LF images and viewport adaptive 360 images as illustrative applications, and I-, P- and previously proposed merge frames to intra- and inter-code MDUs, we show experimentally that landmarked MDU structures can noticeably reduce the expected transmission cost compared with MDU structures without landmarks.

==> problem.tex <==
%Given I- and P- frames coded using HEVC \cite{sullivan2012overview} and M-frames coded using  \cite{dai2016merge}---all at a sufficiently fine pre-fixed quantization parameter (QP) for a target image quality, 
%Given HD media can be encoded with specific techniques according to the media type, 
We focus now on the problem to determine which P-MDUs to be pre-encoded to minimize the expected transmission cost given a storage constraint.
For a given MDU structure $\Theta$, we define the storage cost $b(\Theta)$ as the total size of all the pre-encoded differential P-MDUs:
\begin{eqnarray}
b(\Theta) = \sum \limits_{P_j(i) \in \Theta} |P_j(i)|
\label{eq:storage}
\end{eqnarray}
where $|P_j(i)|$ is the coding bit-rate of P-MDU $P_j(i)$. 
I- and M-MDUs are not considered since they are pre-encoded by default into the structure $\Theta$.

Having defined the expected transmission cost and the storage cost for a given structure $\Theta$,
% we use Lagrange relaxation to find the frame structure that optimally trades off the expected transmission cost and the storage cost, \textit{i.e.}, 
we can now define the optimal MDU structure design problem: find a structure $\Theta^*$ that optimally trades off the expected transmission cost and storage cost, \textit{i.e.}
\begin{eqnarray}
\Theta^* = \arg \min \limits_\Theta c(\Theta) + \lambda b(\Theta).
\label{eq:object}
\end{eqnarray}
where $\lambda$ is a parameter trading off expected transmission cost with storage cost.
In the case of the fixed one-MDU reference buffer, expected transmission cost $c(\Theta) = c_s^{(0)}$ is computed using (\ref{eq:objFixed2}) given $\Theta$. 
In the case of the flexible one-MDU reference buffer, it is computed using (\ref{eq:objFlex}).
%In the case for the fixed one-MDU reference buffer, $c(\Theta) = c_s^{(0)}$ is the expected transmission cost computed by (\ref{eq:objFixed2}) for a given MDU structure $\Theta$ starting from an initial MDU $s$. 
%In the case for the flexible one-MDU reference buffer, $c(\Theta) = c_s^{(0)}(\emptyset)$ is computed by (\ref{eq:objFlex}) given $\Theta$.

